Faithful or Extractive? On Mitigating the Faithfulness-Abstractiveness Trade-off in Abstractive Summarization

Despite recent progress in abstractive summarization, systems still suffer from faithfulness errors. While prior work has proposed models that improve faithfulness, it is unclear whether the improvement comes from an increased level of extractiveness of the model outputs as one naive way to improve faithfulness is to make summarization models more extractive. In this work, we present a framework for evaluating the effective faithfulness of summarization systems, by generating a faithfulnessabstractiveness trade-off curve that serves as a control at different operating points on the abstractiveness spectrum. We then show that the Maximum Likelihood Estimation (MLE) baseline as well as a recently proposed method for improving faithfulness, are both worse than the control at the same level of abstractiveness. Finally, we learn a selector to identify the most faithful and abstractive summary for a given document, and show that this system can attain higher faithfulness scores in human evaluations while being more abstractive than the baseline system on two datasets. Moreover, we show that our system is able to achieve a better faithfulness-abstractiveness trade-off than the control at the same level of abstractiveness.

==> conclusion.tex <==
\section{Conclusion}

\km{I feel like you could reduce implications and use it as conclusions instead. This paragraph does not add much new. Or you could use this paragraph to start and then add in what's new from implications. }\hh{Agree on merging implication and conclusion.}

In this work, we show the relationship between 
faithfulness and extractiveness. We present a measure of ``effective faithfulness'' that allows us to compare models to the baseline at the similar level of abstractiveness. We show that existing models are not able to achieve a better faithfulness-abstractiveness trade-off than the baseline models. We then presented selector models that improve this trade-off. We suggest the community to use this notion of effective faithfulness to make progress in building more abstractive and faithful summarization systems. 
